Zero Grads: Learning Local Surrogate Losses for Non-Differentiable Graphics

Gradient-based optimization is now ubiquitous across graphics, but unfortunately can not be applied to problems with undefined or zero gradients. To circumvent this issue, the loss function can be manually replaced by a ``surrogate'' that has similar minima but is differentiable. Our proposed framework, ZeroGrads, automates this process by learning a neural approximation of the objective function, which in turn can be used to differentiate through arbitrary black-box graphics pipelines. We train the surrogate on an actively smoothed version of the objective and encourage locality, focusing the surrogate's capacity on what matters at the current training episode. The fitting is performed online, alongside the parameter optimization, and self-supervised, without pre-computed data or pre-trained models. As sampling the objective is expensive (it requires a full rendering or simulator run), we devise an efficient sampling scheme that allows for tractable run-times and competitive performance at little overhead. We demonstrate optimizing diverse non-convex, non-differentiable black-box problems in graphics, such as visibility in rendering, discrete parameter spaces in procedural modelling or optimal control in physics-driven animation. In contrast to other derivative-free algorithms, our approach scales well to higher dimensions, which we demonstrate on problems with up to 35k interlinked variables.

==> integrals.tex <==
E_x[F(x, E_y[G(y,x)])]
E_x[x - E_y[G(y,x)]]
E_x[E_y[x] - E_y[G(y,x)]]
E_x[E_y[x - G(y,x)]]
E_x[E_y[F(x, G(y,x)])]

int_x[F(x, int_y[G(y,x)]dy)]dx
int_x[x - int_y[G(y,x)]dy]dx
int_x[int_y[x]dy - int_y[G(y,x)]dy]dx
int_x[int_y[x - G(y,x)]dy]dx
int_x[int_y[F(x, G(y,x)])]dydx

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> tr-acronyms.tex <==
\acro{AD}{automatic differentiation}
\acro{BN}{batch normalization}
\acro{BRDF}{bi-directional reflectance distribution function}
\acro{BTF}{bi-directional texture function}
\acro{CNN}{convolutional neural network}
\acro{DA}{dual annealing}
\acro{DGS}{directional Gaussian smoothing}
\acro{DSSIM}{structural dissimilarity}
\acro{FD}{finite differences}
\acro{GA}{genetic algorithm}
\acro{GD}{gradient descent}
\acro{IOR}{index of refraction}
\acro{KL}{Kullback-Leibler}
\acro{KLD}{Kullback-Leibler divergence}
\acro{LHS}{Latin hypercube sampling}
\acro{MAE}{mean absolute error}
\acro{MASA}{mixed adaptive sampling algorithm}
\acro{MC}{Monte Carlo}
\acro{MCMC}{Markov-chain Monte Carlo}
\acro{ML}{machine learning}
\acro{MLP}{multi-layered perceptron}
\acro{MSE}{mean-squared error}
\acro{NAS}{neural architecture search}
\acro{NeRF}{neural radiance fields}
\acro{NN}{neural network}
\acro{NLL}{negative $\log$-likelihood}
\acro{NP}{neural proxy}
\acro{ODE}{ordinary differential equation}
\acro{PCA}{principal component analysis}
\acro{QMC}{quasi-Monte Carlo}
\acro{PDF}{probability density function}
\acro{RBF}{radial basis function}
\acro{RSM}{response surface map}
\acro{SA}{simulated annealing}
\acro{SPSA}{simultaneous perturbation stochastic approximation}
\acro{SDF}{signed distance function}
\acro{SSIM}{structural similarity}
\acro{svBRDF}{spatially-varying BRDF}
\acro{VAE}{variational autoencoder}



==> tr-math.tex <==
\mymath{\adjoint}a
\mymath{\lossOffset}{\rho}
\mymath{\learningRate}{\alpha}
\mymath{\locality}{\lambda}
\mymath{\mcmcSample}{y}
\mymath{\mcmcSampleGradient}{\mathbf z}
\mymath{\mcmcState}{\bar}
\mymath{\objective}f
\mymath{\offset}{\tau}
\mymath{\parameters}{\theta}
\mymath{\parameterDimension}n
\mymath{\parameterSpace}{\Theta}
\mymath{\sampleCount}{N}
\mymath{\smoothObjective}g
\mymath{\smoothingKernel}{\kappa}
\mymath{\spreadinner}{\sigma_i}
\mymath{\spreadouter}{\sigma_o}
\mymath{\surrogate}h
\mymath{\surrogateLoss}l
\mymath{\surrogateParameters}{\phi}
\mymath{\surrogateParameterSpace}{\Phi}
\mymath{\surrogateParameterDimension}m
\mymath{\potentialMatrix}{\textsf{M}}
\mymath{\inputvector}{\textrm{x}}


% for experiments: 
\mymath{\nsplinepts}{10}
\mymath{\numtexels}{196,608}
\mymath{\texturedim}{256}
\mymath{\numvertices}{2,562}
\mymath{\meshdim}{7,686}
\mymath{\numweights}{35,152}
\mymath{\numsplineweights}{8,764}
